Sparse Mutation Decompositions: Fine Tuning Deep Neural Networks with Subspace Evolution

Neuroevolution is a promising area of research that combines evolutionary algorithms with neural networks. A popular subclass of neuroevolutionary methods, called evolution strategies, relies on dense noise perturbations to mutate networks, which can be sample inefficient and challenging for large models with millions of parameters. We introduce an approach to alleviating this problem by decomposing dense mutations into low-dimensional subspaces. Restricting mutations in this way can significantly reduce variance as networks can handle stronger perturbations while maintaining performance, which enables a more controlled and targeted evolution of deep networks. This approach is uniquely effective for the task of fine tuning pre-trained models, which is an increasingly valuable area of research as networks continue to scale in size and open source models become more widely available. Furthermore, we show how this work naturally connects to ensemble learning where sparse mutations encourage diversity among children such that their combined predictions can reliably improve performance. We conduct the first large scale exploration of neuroevolutionary fine tuning and ensembling on the notoriously difficult ImageNet dataset, where we see small generalization improvements with only a single evolutionary generation using nearly a dozen different deep neural network architectures.

==> notes.tex <==
The Lottery Ticket Hypothesis: Finding Sparse, Trainable Neural Networks (2019)
https://arxiv.org/abs/1803.03635

Frankle et al set out to explore the learning dynamics of sparse networks in a popular paper called The Lottery Ticket Hypothesis. They found that randomly initialized sparse networks are unable to match the performance of the original networks. However, they were able to find high performing sparse networks by training a full network, iteratively pruning the lowest magnitude weights, and rewinding the pruned network to the original weight initializations. These high performing subnetworks are thought to be winners of the weight initialization lottery, and they often match and outperform their dense counterparts.

An interesting finding in their work is that they were unable to find winning tickets in larger, modern architectures (VGG19 and Resnet18) with standard initial learning rates (0.1).

---

Stabilizing the Lottery Ticket Hypothesis (2019)
https://arxiv.org/abs/1903.01611

This paper is a followup to the original lottery ticket hypothesis. They aim to address the small scale limitations of the original work. The primary idea they explore is instead of rewinding to the original weight values, you instead rewind the ticket to the weights at iteration k.

They find that you can successfully prune up to 85\% of the weights while still matching the full size test performance. With this approach, they are able to find subnetworks without modifying learning rates. As the initial weights are rewound to values after k iterations of training, the subnetworks are then called "matching tickets" rather than lottery tickets.

---

(2020) Comparing Rewinding and Fine-tuning in Neural Network Pruning
https://arxiv.org/abs/2003.02389

This paper compares the lottery ticket procedure, which includes both weight and learning rate rewinding with fine-tuning. 

On Resnet, they found that weight rewinding and retraining outperforms simple fine tuning in both unlimited and fixed budget experiments.

They also found that learning rate rewinding outperforms weight rewinding.

---

Deconstructing Lottery Tickets: Zeros, Signs, and the Supermask (2019)
https://papers.nips.cc/paper/2019/file/1113d7a76ffceca1bb350bfe145467c6-Paper.pdf

This paper set out to explore what the main ingredients in determining a winning ticket is.

What is special about the pruning criteria?
Lottery ticket keeps the largest magnitude trained weights. This paper explores the smallest trained weights, the largest/smallest weights at initialization, and the magnitude change/movement in the weight space.

What about other rewinding strategies?
Random reinitialization, reshuffling the kept weights, and a constant initialization.

What if pruning weights by freezing at 0, what if we freeze the weights other values?
They explore setting pruned weights to their initial values and freezing there.

Keeping weights with largest magnitude increase performs even better than largest final weights. Everything else is worse than these two. They found that randomly reinitializing the weights but keeping the same sign works as well as rewinding. This finding was not able to be replicated in future work. And masking the weights to 0 performs much better than freezing weights to their initial value.

They conclude that pruning and informed masking can be viewed as a form of training. It accelerates the trajectory of the weights that were already heading towards 0.

---

Linear Mode Connectivity and the Lottery Ticket Hypothesis
https://arxiv.org/abs/1912.05671

This paper explores SGD noise. Notably the random ordering of data batches during trianing. Imagine a single set of initial weights that is trained on two seperate random data orders. We might end up with very different final weights. This paper explores how these final weights are related by interpolating between these final weight configurations. They call networks stable if the error does not increase significantly between interpolations of these final networks.

They find that the stability of networks is related to the iteration k you have to roll back to. They find that lottery tickets (Iterative Magnitude Pruning) induces stability. According to the amount of pruned weights, there are 3 regimes. At small amounts of pruning, any pruning method results in good performance. At medium-high amounts of pruning, only IMP yields matching and stable tickets. At extreme pruning, IMP can yield stable networks but no longer matching tickets.

---

The Early Phase of Neural Network Training
https://openreview.net/forum?id=Hkl1iRNFwS

This paper aims to explore the robustness of matching tickets. How much can you perturb the initializations before the lottery tickets lose their ability to perform?

Perturbations include:

Combining the magnitude at time point x with the signs at time point y.

Permute the weights at iteration k with subcomponents of the net. Exchanging the weights globally across layers, locally within layers, and locally within filters.

Add gaussian noise to the matching ticket weights.

Pretraining with different self supervised losses.


They conclude that it is hard to overcome the necessity of using rewinding, since the emergence of the matching initialization is non-trivial. Self supervised pretraining may be a potential way to circumvent rewinding.

---

Drawing early-bird tickets: Towards more efficient training of deep networks
https://arxiv.org/abs/1909.11957

Finding tickets is costly. You still need to fully and iteratively train and prune. This paper aims to find winning tickets early in training.

They do this by combining early stopping with low precision and large learning rates. They argue that there is two phases in optimization.

1. A robust phase of learning large singular value components.
2. An absorbing phase of learning small singular value components.

They find that pruning masks change significantly during the first epochs of training, but appear to converge soon.

---

Pruning neural networks without any data by iteratively conserving synaptic flow
https://arxiv.org/abs/2006.05467

They argue the biggest challenge to pruning it initialization is the problem of layer collapse. That pruning to much of a layer can render much of the architecture untrainable since the gradient flow is cut off.

They show that typical gradient based pruning methods result in layer collapse for significant pruning. But, IMP tends to preserve gradient flow. They suggest that gradient descent encourges layer wise conservation.

They suggest an algorithm for pruning that maintains layer-wise synaptic flow that does not require training data and it outperforms other pruning-at-init baselines.

---

One ticket to win them all: generalizing lottery ticket initializations across datasets and optimizers
https://arxiv.org/abs/1906.02773

Are lottery tickets overfit?

Find a lottery ticket on a source dataset. Evaluate the lottery ticket on a new target dataset.

They find that the transferred tickets from cifar to imagenet perform well, but worse than a ticket found on directly on imagenet. Tickets transferred from imagenet to cifar perform even better than one inferred from cifar.

They also investigate transfer of optimizers (adam, rmsprop, sgd). They find that they can transfer with carefully tuned learning rates.


---

The State of Sparsity in Deep Neural Networks
https://arxiv.org/abs/1902.09574

They found that no pruning method trained from scratch performs as well as methods that induce sprarsity throughout training.

Also,

"Additionally, we provide strong counterexamples to two recently proposed theories that models learned through pruning techniques can be trained from scratch to the same test
set performance of a model learned with sparsification as
part of the optimization process."

---

Rethinking the Value of Network Pruning
https://arxiv.org/abs/1810.05270

"We also compare with the "Lottery Ticket Hypothesis" (Frankle & Carbin 2019), and find that with optimal learning rate, the "winning ticket" initialization as used in Frankle & Carbin (2019) does not bring improvement over random initialization."

---

Gradient Flow in Sparse Neural Networks and How Lottery Tickets Win
https://arxiv.org/pdf/2010.03533.pdf

Sparse NNs have poor gradient flow at initialization and during training. Lottery Tickets don't improve on gradient flow. 

They merely re-learn the solution they were pruned from. That is, a lottery ticket lies in the same "basin of attraction" as whatever solution was found with the full network. Investigate perturbations to lottery ticket subnetworks. They find they are robust to all perturbations as long as the resulting network lies within the basin of attraction.

---

Rigging the Lottery: Making All Tickets Winners
https://arxiv.org/abs/1911.11134

A sparse training algorithm.

Start with random sparse topology.

At regularly spaced intervals, remove a fraction of the connections with the smallest magnitudes and activate new connections using current gradient information.

Continue training and repeat.

---

Pruning neural networks at initialization: What are we missing?
https://openreview.net/pdf?id=Ig-VyQc-MLK

In depth comparison of current pruning methods. Lottery Tickets, Snip, Grasp, Synflow, Magnitude. While these methods do improve over random pruning, none of the pruning methods at initialization competes with pruning after training. Knowing a "final" solution is the only reason lottery tickets work. And even then, lottery tickets only work best with rewinding to state k.

They also investigate several ablations with pruned networks. Reinitialization. Shuffling weights. Inverting weights.

Supports our point. There is no magic subnetwork at initialization.

---

Proving the Lottery Ticket Hypothesis
http://proceedings.mlr.press/v119/malach20a/malach20a.pdf

The lottery ticket hypothesis states that a randomly-initialized network contains a small subnetwork such that, when trained in isolation, can compete with the performance of the original network. We prove an even stronger hypothesis (as was also conjectured in Ramanujan et al., 2019), showing that for every bounded distribution and every target network with bounded weights, a sufficiently over-parameterized neural network with random weights contains a subnetwork with roughly the same accuracy as the target network, without any further training.

---

What's hidden in a randomly weighted neural network?
https://arxiv.org/abs/1911.13299

Builds on the supermask idea. There's subnetworks in large enough networks that perform well with no weight training. They demonstrate a subnetwork in resnet50 that achieves comparable performance to resnet34 with no training.

"To this end we propose the edge-popup algorithm
for finding effective subnetworks within randomly weighted
neural networks. We show a significant boost in performance and scale to ImageNet. For each fixed random
weight in the network, we consider a positive real-valued
score. To choose a subnetwork we take the weights with
the top-k% highest scores. With a gradient estimator we
optimize the scores via SGD. We are therefore able to find
a good neural network without ever changing the values of
the weights. We empirically demonstrate the efficacy of our
algorithm and show that (under certain technical assumptions) the loss decreases on the mini-batch with each modification of the subnetwork."

---

INTRO NOTES

The problem is that evolutionary methods have not shown much success in supervised learning with extremely high dimensional models like deep neural networks.


Evolution strategies are a class of black-box search algorithms that are inspired by biological evolution. They often use analogous evolutionary operations like mutation, selection, and recombination in order to optimize a set of parameters over time according to some fitness score. They are known to be highly scalable, but sample inefficient. 

They have seen the most success in reinfocement learning, as they excel at finding diverse solutions and avoiding local minima that a gradient based method might fall in to.


Evolutionary methods scale well on small problems with small models as they avoid local minima that gradient methods would be prone to getting stuck in. However, evolutionary methods are sample inefficient and struggle with high dimensional models like deep neural networks. Therefore, they have not shown much success with supervised learning and computer vision. 

Generally evolutionary learning optimizes a single set of parameters and returns a single classifier. However, the population can instead be framed as an ensemble for free. Ensemble learning is a reliable and consistent way to improve generalization performance.


Evolutionary Strategies is a class of black-box search algorithms that use mechanisms inspired by biological evolution. A core component of evolutionary strategies is the generation of a population of members as a result of perturbative {\it mutations}. These members are evaluated individually, and the fitness of each forms a surrogate gradient that is used to optimize a set of parameters. 



In the context of neural networks, this is generally done with random noise generated from a gaussian process. This approach has shown to be successful in simple reinforcement learning environments, using models with a small number of parameters. However, the sample inefficiency and intractability of pseudo-random search in high dimensional spaces on the scale of deep neural networks, has prevented this approach from seeing much success in computer vision and supervised learning.

Evolutionary Strategies excel at finding diverse solutions, as they are less likely to settle into local optima and they are extremely parallel, which makes scaling the number of members in a population trivial. However, these methods tend to be terribly sample inefficient and intractable for models of high dimensionality.


Ensembles of neural networks are a reliable and consistent way to improve generalization. We aim to explore evolutionary populations in the context of deep neural networks. We show that simple noise perturbations can improve the generalization of fully trained deep neural networks, {\it with no additional training}.

Motivations: Call out to this idea behind SWA. Networks generally converge to the edges of wide minima. These are places that the training distribution likely {\it slightly} differs from the test distributions. Ensembling over this small area improves generalization.
